Expectation-Maximization Based Defense Mechanism for Distributed Model Predictive Control

Controlling large-scale systems sometimes requires decentralized computation. Communication among agents is crucial to achieving consensus and optimal global behavior. These negotiation mechanisms are sensitive to attacks on those exchanges. This paper proposes an algorithm based on Expectation Maximization to mitigate the effects of attacks in a resource allocation based distributed model predictive control. The performance is assessed through an academic example of the temperature control of multiple rooms under input power constraints.

==> article.aux.1 <==
\relax 
\bibstyle{ifacconf}
\citation{KantamneniEtAl2015}
\citation{MaestreEtAl2014}
\citation{VelardeEtAl2017}
\citation{ChanfreutEtAl2018}
\citation{NogueiraEtAl2021}
\citation{VelardeEtAl2017}
\citation{MaestreEtAl2021}
\citation{NogueiraEtAl2021}
\citation{DempsterEtAl1977}
\newlabel{First}{{*\relax }{1}}
\global\@namedef{n@author@}{4}
\global\@namedef{n@collab@}{0}
\providecommand \oddpage@label [2]{}
\providecommand\@newglossary[4]{}
\@newglossary{main}{glg}{gls}{glo}
\@newglossary{acronym}{alg}{acr}{acn}
\@writefile{toc}{\contentsline {section}{\numberline {1}INTRODUCTION}{1}{}\protected@file@percent }
\citation{BoydEtAl2015}
\citation{BoydEtAl2015}
\citation{NogueiraEtAl2021}
\@writefile{toc}{\contentsline {section}{\numberline {2}Problem Statement}{2}{}\protected@file@percent }
\newlabel{sec:PS}{{2}{2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.1}Model Predictive Control}{2}{}\protected@file@percent }
\newlabel{ssec:MPC}{{2.1}{2}}
\newlabel{eq:systems}{{1}{2}}
\newlabel{eq:u_local_constraints}{{2}{2}}
\newlabel{eq:global_constraint}{{3}{2}}
\newlabel{eq:GOP}{{4}{2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.2}Primal Decomposition based dMPC}{2}{}\protected@file@percent }
\newlabel{ssec:dMPC}{{2.2}{2}}
\newlabel{eq:DOP_local}{{5a}{2}}
\newlabel{eq:DOP_master}{{5b}{2}}
\newlabel{eq:projectedSubgradient}{{6}{2}}
\newlabel{eq:thetaNegot}{{7}{2}}
\@writefile{loa}{\contentsline {algocf}{\numberline {1}{\ignorespaces Quantity decomposition based \acrshort {dmpc}.}}{3}{}\protected@file@percent }
\newlabel{alg:quantityAlg}{{1}{3}}
\@writefile{toc}{\contentsline {section}{\numberline {3}Towards a safe dMPC}{3}{}\protected@file@percent }
\newlabel{sec:TSM}{{3}{3}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1}Local Problems --- Formal Analysis}{3}{}\protected@file@percent }
\newlabel{ssec:FA}{{3.1}{3}}
\newlabel{eq:quadratic_case}{{8}{3}}
\newlabel{eq:4}{{8a}{3}}
\newlabel{eq:constraints}{{8b}{3}}
\newlabel{eq:lambdafuntheta}{{9}{3}}
\newlabel{rmk:P_constant}{{1}{3}}
\newlabel{ch:zone_unknown}{{1}{3}}
\newlabel{ch:s_unknown}{{2}{3}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Exchange between coordinator and agents.}}{3}{}\protected@file@percent }
\newlabel{fig:dmpc_graph}{{1}{3}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2}The Attack}{3}{}\protected@file@percent }
\newlabel{ssec:attack}{{3.2}{3}}
\newlabel{eq:linear_cheating}{{11}{3}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.3}Detection and mitigation}{3}{}\protected@file@percent }
\newlabel{ssec:DM}{{3.3}{3}}
\newlabel{eq:lambdafuntheta_tilde}{{12}{3}}
\newlabel{ass:Pnominal}{{4}{3}}
\newlabel{eq:2}{{13}{3}}
\citation{FariaSoromenho2010}
\citation{ChristensenEtAl2010}
\citation{Bishop2006}
\citation{OzerovFevotte2010}
\newlabel{eq:lambda_reconstruction}{{15}{4}}
\newlabel{ass:}{{6}{4}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.4}Expectation Maximization}{4}{}\protected@file@percent }
\newlabel{eq:m_step}{{16}{4}}
\@writefile{loa}{\contentsline {algocf}{\numberline {2}{\ignorespaces Expectation Maximization}}{4}{}\protected@file@percent }
\newlabel{alg:em}{{2}{4}}
\newlabel{eq:linear_cheating_random}{{17}{4}}
\newlabel{eq:multivariate_gaussian}{{18}{4}}
\newlabel{eq:responsibilities}{{19}{4}}
\newlabel{eq:completedataLogLikelihood_expectation}{{20}{4}}
\newlabel{eq:mstepestimation}{{21}{4}}
\citation{BradleyMangasarian2000}
\citation{Bishop2006}
\citation{NogueiraEtAl2021}
\newlabel{eq:3}{{3.4}{5}}
\newlabel{eq:argmaxz}{{3.4}{5}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.5}Safe dMPC Algorithm}{5}{}\protected@file@percent }
\newlabel{ssec:safe_algo}{{3.5}{5}}
\@writefile{loa}{\contentsline {algocf}{\numberline {3}{\ignorespaces Secure DMPC.}}{5}{}\protected@file@percent }
\newlabel{alg:safeDMPC}{{3}{5}}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Exchange between agents in secure \gls {dmpc}{}.}}{5}{}\protected@file@percent }
\newlabel{fig:safe_dmpc_graph}{{2}{5}}
\@writefile{toc}{\contentsline {section}{\numberline {4}Example: Temperature Control}{5}{}\protected@file@percent }
\newlabel{sec:App_dMPC}{{4}{5}}
\newlabel{eq:systems_cont}{{22}{5}}
\newlabel{eq:room_system}{{4}{5}}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces Model Parameters}}{5}{}\protected@file@percent }
\newlabel{tab:modelParamMeaning}{{1}{5}}
\@writefile{lot}{\contentsline {table}{\numberline {2}{\ignorespaces  Parameters for each agent}}{5}{}\protected@file@percent }
\newlabel{tab:modelParam}{{2}{5}}
\bibdata{bibliography}
\bibcite{Bishop2006}{{1}{2006}{{Bishop}}{{}}}
\bibcite{BoydEtAl2015}{{2}{2015}{{Boyd et~al.}}{{Boyd, Xiao, Mutapcic, and Mattingley}}}
\bibcite{BradleyMangasarian2000}{{3}{2000}{{Bradley and Mangasarian}}{{}}}
\bibcite{ChanfreutEtAl2018}{{4}{2018}{{{Chanfreut} et~al.}}{{{Chanfreut}, {Maestre}, and {Ishii}}}}
\bibcite{ChristensenEtAl2010}{{5}{2010}{{Christensen et~al.}}{{Christensen, Johnson, Branscum, and Hanson}}}
\bibcite{DempsterEtAl1977}{{6}{1977}{{Dempster et~al.}}{{Dempster, Laird, and Rubin}}}
\bibcite{FariaSoromenho2010}{{7}{2010}{{Faria and Soromenho}}{{}}}
\bibcite{KantamneniEtAl2015}{{8}{2015}{{Kantamneni et~al.}}{{Kantamneni, Brown, Parker, and Weaver}}}
\bibcite{MaestreEtAl2014}{{9}{2014}{{Maestre et~al.}}{{Maestre, Negenborn et~al.}}}
\bibcite{MaestreEtAl2021}{{10}{2021}{{Maestre et~al.}}{{Maestre, Velarde, Ishii, and Negenborn}}}
\bibcite{NogueiraEtAl2021}{{11}{2021}{{Nogueira et~al.}}{{Nogueira, Bourdais, and Gu{\'e}guen}}}
\bibcite{OzerovFevotte2010}{{12}{2010}{{Ozerov and Fevotte}}{{}}}
\bibcite{VelardeEtAl2017}{{13}{2017}{{Velarde et~al.}}{{Velarde, Maestre, Ishii, and Negenborn}}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces Air temperature in room I and the decision variable $E_{I}[k]$ for different scenarios: nominal (N), selfish behavior without correction (S), and selfish behavior with correction.}}{6}{}\protected@file@percent }
\newlabel{fig:response3Scenarios}{{3}{6}}
\@writefile{lot}{\contentsline {table}{\numberline {3}{\ignorespaces Comparison of objective functions $J$}}{6}{}\protected@file@percent }
\newlabel{tab:costsGlobalLocal}{{3}{6}}
\@writefile{toc}{\contentsline {section}{\numberline {5}CONCLUSION AND FUTURE WORKS}{6}{}\protected@file@percent }
\newlabel{sec:CC}{{5}{6}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces Control applied in all rooms for the 3 scenarios.}}{6}{}\protected@file@percent }
\newlabel{fig:control_3Scenarios}{{4}{6}}
\global\c@lastpage=7
\global\NAT@numbersfalse
\gdef \@abspage@last{7}


==> makefile <==
OBJ=article

all: $(OBJ).pdf

$(OBJ).pdf: $(OBJ).tex $(OBJ).bbl
	@echo PDF
	@pdflatex -interaction errorstopmode -synctex=1 $(OBJ).tex >/dev/null
	@pdflatex -interaction errorstopmode -synctex=1 $(OBJ).tex >/dev/null

$(OBJ).aux.1: $(OBJ).tex
	@echo CREATING AUX FILE
	@pdflatex  -interaction nonstopmode $(OBJ).tex >/dev/null
	@cp $(OBJ).aux $(OBJ).aux.1

$(OBJ).cites: $(OBJ).aux.1
	@echo VERIFYING CITATIONS
	@grep citation $(OBJ).aux.1 | sort > $@.1
	@touch $@.1
	@if [ ! -f "$@" ]; then touch $@; fi
	@if [ "`diff -N $@ $@.1`" != "" ];\
	then \
	echo " CITATIONS CHANGED";\
	cp $@.1 $@ ;\
	fi;
	@rm -f $@.1;
	@if [ -f "$@" ]; then touch $< -r $@; fi
	@if [ -f "$@" ]; then touch $(OBJ).tex -r $@; fi

$(OBJ).bbl: $(OBJ).cites bibliography.bib
	@echo BIBTEX
	@if [ "`diff -N $(OBJ).cites ""`" != "" ];\
	then bibtex $(OBJ) >/dev/null;\
	if [ "`grep bibitem $(OBJ).bbl`" = "" ];\
	then echo NO CITATION FOUND;\
	echo " " > $(OBJ).bbl;\
	fi;\
	else echo " " > $(OBJ).bbl;\
	fi


view: $(OBJ).pdf
	zathura $(OBJ).pdf&

detex: $(OBJ)_detexed.tex
$(OBJ)_detexed.tex: $(OBJ).tex
	detex -n -r -e "array,eqnarray,equation,longtable,table,picture,tabular,verbatim,usetikzlibrary" $(OBJ) > $@

clean:
	@rm -rf  $(OBJ).aux.1 $(OBJ).aux $(OBJ).out $(OBJ).log
	@rm -rf  $(OBJ).synctex.gz $(OBJ).upa $(OBJ).upb
	@rm -rf  $(OBJ).ist $(OBJ).acn $(OBJ).glsdefs $(OBJ).glo
	@rm -rf  $(OBJ).cites $(OBJ).bbl $(OBJ).blg $(OBJ).bcf

clean-all: clean
	@rm -rf $(OBJ).pdf


==> table_costs_only_global.tex <==
Global & $ 112770.6 $ ($ 0.0 $)& $ 125614.4 $ ($ 10.0 $)& $ 112770.6 $ ($ -0.0 $)

